Efficient Amortised Bayesian Inference for Hierarchical and Nonlinear Dynamical Systems

We introduce a flexible, scalable Bayesian inference framework for nonlinear dynamical systems characterised by distinct and hierarchical variability at the individual, group, and population levels. Our model class is a generalisation of nonlinear mixed-effects (NLME) dynamical systems, the statistical workhorse for many experimental sciences. We cast parameter inference as stochastic optimisation of an end-to-end differentiable, block-conditional variational autoencoder. We specify the dynamics of the data-generating process as an ordinary differential equation (ODE) such that both the ODE and its solver are fully differentiable. This model class is highly flexible: the ODE right-hand sides can be a mixture of user-prescribed or "white-box" sub-components and neural network or "black-box" sub-components. Using stochastic optimisation, our amortised inference algorithm could seamlessly scale up to massive data collection pipelines (common in labs with robotic automation). Finally, our framework supports interpretability with respect to the underlying dynamics, as well as predictive generalization to unseen combinations of group components (also called "zero-shot" learning). We empirically validate our method by predicting the dynamic behaviour of bacteria that were genetically engineered to function as biosensors. Our implementation of the framework, the dataset, and all code to reproduce the experimental results is available at https://www.github.com/Microsoft/vi-hds .

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> stuff_for_figures.tex <==


\begin{align*}
    \vz = \vz_{\glob} \cup \vz_{\local} \cup  \vz_{\device} \\
    \vz_{\glob} \sim \qdist_{\glob}( \vmu_{\glob}, \msigma_{\glob} )\\
    \vz_{\device} \sim \qdist_{\device}( \vmu_{\device}( \vdevice ), \msigma_{\device}( \vdevice ) )\\
    \vz_{\local} \sim \qdist_{\local}( \vmu_{\local}( \vobs, \vdevice ), \msigma_{\local}( \vobs, \vdevice ) )
\end{align*}

\begin{align*}
    \dfrac{d\vx}{dt} &= f( \vx, \vz, \vdevice, \vtreat) \\
    \vobsest &= g(\vx) \\
    \mobs &= \left[ \vobs_1, \ldots, \vobs_{T} \right] \\
    \mobsest &= \left[ \vobsest_1, \ldots, \vobsest_{T} \right] \\
    \mx &= \left[ \vx_1, \ldots, \vx_{T} \right] \\
    \mobsest &= g(\mx) \\
     p( \mobs | \mobsest ) &= h( \mobs, \mobsest, \mx, \vz )
\end{align*}

\subsection{Notation Work}

\paragraph{Devices} A device is defined as the composition of $\nsubs$ sub-components called cassettes and each cassette $\devicecomp_{\devicesub}$ belongs to $1$ of $\ndevicesub$ variations.  We represent device sub-components $\vdevice^{(\devicesub)}$ as $\ndevicesub$-dimensional one-hot vectors, where: 
\[ \vdevice^{(\devicesub)}_{\subidx} =
  \begin{cases}
    1       & \quad \text{if } \devicecomp_{\devicesub} = \subidx \\
    0  & \quad \text{otherwise} 
  \end{cases}
\]
and an entire device as the concatenation of $\nsubs$ device sub-components:
\begin{align*}
    \vdevice &= \left[ \vdevice^{(1)T}, \vdevice^{(2)T}, \ldots, \vdevice^{(\nsubs)T} \right]^T
\end{align*}
The device for a data instance $\dataidx$ is indicated by $\vdevice_{\dataidx}$, and the entire matrix of devices is $\mdevice = \left[ \vdevice_1^T, \vdevice_1^T, \ldots,  \vdevice_{\ndata}^T \right]^T$.
In our synthetic biology application $\nsubs=2$ and represent promoters which activate yellow and cyan fluorescent proteins.  In general though the device represents additional observations that is known both at train and test time, but could easily be extended to semi-supervised scenarios.

\paragraph{Treatments} A treatment $\vtreat$ is a $\ntreatments$ vector representing the concentrations of chemicals applied to a bacteria colony during the course of the experiment.  In general the treatment can be viewed as the experimental conditions for a given experimental set-up, here being the bacterial colony having a specific device composition.  The treatment for a data instance $\dataidx$ is indicated by $\vtreat_{\dataidx}$, and the entire matrix of treatments is $\mtreat = \left[ \vtreat_1^T, \vtreat_2^T, \ldots,  \vtreat_{\ndata}^T \right]^T$.  In our application, $\ntreatments = 2$, representing the concentrations of HSL \tedcomment{HSL?} signals $C_6$ and $C_{12}$.  

\paragraph{Time-series Observations} Each data instance $\dataidx$ has $\nspecies$ observed times-series each of length $\ntime$, which we represent as a $\nspecies \times \ntime$-dimensional matrix $\mobs_{\dataidx}$. Observations at a single time-instance will be $\nspecies$ vectors $\vobs$, so that $\mobs = \left[ \vobs_1, \ldots, \vobs_{\ntime} \right]$; note $\vobs \geq 0$. 
In our application $\nspecies = 4$, representing the optical density (OD), bulk red fluorescence (RFP), bulk yellow fluorescence (YFP), and bulk cyan fluorescence (CYP). 

\subsection{old}

\tedcomment{Recommend a paragraph on notation, which can explain the experimental data too.  Need to change treatments to vector notation, write devices not as one-hot over all devices, but over composition of one-hot cassettes.}
\subsection{Notation and Experimental Data}
Each input datum $\mathbf{y}^{(i)}$ is a $(4 \times T)$ vector in $\mathbb{R}_{\geq 0}$ corresponding to $T$ observations of each of the optical density (OD), bulk yellow flourescence (YFP), bulk cyan flourescence (CFP), and bulk red flourescence (RFP) of a bacterial colony.
The $N$ observed datapoints are collected in the tensor $\vy \in \mathbb{R}_{\geq 0}^{N \times 4 \times T}$, $N$ observations of a time series with $4$ channels and $T$ steps in the evolution of the process.
OD correlates strongly with the current size of the engineered bacterial colony. 
The biological circuit that causes the colony to express RFP is constant across all bacterial colonies, and correlates strongly with the baseline metabolic rate of the colony.
The baseline metabolic rate affects the production of the other two florescent proteins and serves as an important point of comparison between circuits.

The bacterial colony is engineered with a particular biological circuit,  represented by a concatenation of device component identifiers, $\vo \in \{0,1\}^{n_d}$, where $n_d$ is the number of functional subunits of DNA in the device.
For example, the $k^{th}$ observation $\mathbf{y}^{(k)}$ is measured from a biological circuit with device identifier $\mathbf{o}=(1,0,0,1)$, indicating that of the four possible functional subunits of DNA represented by this dataset, the 0th and 3rd subunits are implanted in the bacterial colony.
Such a multi-hot representation, when combined with the mixed effects decomposition of the approximate posterior, supports zero-shot learning of unseen device combinations.


    {\color{red} TODO: description of the epxeirmental setup and jsutification of a mixed effects model. should this be in section 2?}

Each colony was subject to a treatment  $\vu \in \mathbb{R}_{\geq 0}^{n_u}$ where $n_u$ is the number of treatments.
We also have access to device identifiers $\vo \in \{0,1\}^{n_d}$, where $n_d$ is the number of distinct devices, that is, $\vo$ is a one-hot representation over devices. 
Since each biological circuit shares some components with other circuits but not others, we explicitly model this in our a conditional posterior distribution.

\tedcomment{Would be great to compare the meaning of mixed effects and conditional VAE for everyone.}
